SciRerankBench: Benchmarking Rerankers Towards Scientific Retrieval-Augmented Generation with LLMs

Scientific literature question answering is a pivotal step towards new scientific discoveries. Recently, \textit{two-stage} retrieval-augmented generated large language models (RAG-LLMs) have shown impressive advancements in this domain. Such a two-stage framework, especially the second stage (reranker), is particularly essential in the scientific domain, where subtle differences in terminology may have a greatly negative impact on the final factual-oriented or knowledge-intensive answers. Despite this significant progress, the potential and limitations of these works remain unexplored. In this work, we present a Scientific Rerank-oriented RAG Benchmark (SciRerankBench), for evaluating rerankers within RAG-LLMs systems, spanning five scientific subjects. To rigorously assess the reranker performance in terms of noise resilience, relevance disambiguation, and factual consistency, we develop three types of question-context-answer (Q-C-A) pairs, i.e., Noisy Contexts (NC), Semantically Similar but Logically Irrelevant Contexts (SSLI), and Counterfactual Contexts (CC). Through systematic evaluation of 13 widely used rerankers on five families of LLMs, we provide detailed insights into their relative strengths and limitations. To the best of our knowledge, SciRerankBench is the first benchmark specifically developed to evaluate rerankers within RAG-LLMs, which provides valuable observations and guidance for their future development.

==> chapters/1_related.tex <==

\section{Related Work}

% \begin{table}[ht]
% \centering
% \caption{Comparison of SciRerankBench among related datasets, toolkits and benchmarks.}
% \vspace{-2mm}
% \label{tab:compare_benchmark}
% \renewcommand{\arraystretch}{0.7}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cccccccc}
% \toprule
% \textbf{Type} & \textbf{Work} & \textbf{\makecell{Source Data}} & \textbf{Explainability} & \textbf{\makecell{Scientific\\Field}} & \textbf{\makecell{Knowledge\\Level}} & \textbf{\makecell{Rerank\\Oriented}} & \textbf{\makecell{Dataset\\Size}} \\
% \midrule
% \multirow{6}{*}{Dataset} 
%     & NQ~\cite{kwiatkowski2019natural} & Google search log & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & General & \textcolor{red}{\ding{55}} & \makecell{307k (train),\\7.8k (dev/test)} \\ \cmidrule(lr){2-8}
%     & HotpotQA~\cite{yang2018hotpotqa} & Wikipedia & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & General & \textcolor{red}{\ding{55}} & 113k \\ \cmidrule(lr){2-8}
%     & PubMedQA~\cite{jin2019pubmedqa} & PubMed abstracts & \textcolor{green}{\ding{51}} & Bio. & Expert & \textcolor{red}{\ding{55}} & \makecell{1k expert,\\61k unlabeled,\\211k generated} \\
% \midrule
% \multirow{2}{*}{Toolkit} 
%     & FlashRAG~\cite{jin2024flashrag} & Public benchmarks & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & General & \textcolor{green}{\ding{51}} & unknown \\ \cmidrule(lr){2-8}
%     & rankify~\cite{abdallah2025rankify} & Public benchmarks & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & General & \textcolor{green}{\ding{51}} & unknown \\
% \midrule
% \multirow{16}{*}{Bench.}
%     & CRAG~\cite{yang2024crag} & Web search log & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & General & \textcolor{red}{\ding{55}} & 4.4K \\ \cmidrule(lr){2-8}
%     & AGIEval~\cite{zhong2023agieval} & Exams & \textcolor{red}{\ding{55}} & \makecell{Geo., Bio., His.,Chem., Phy.,\\ Eng., Chi., Math, Law, Log.} & High school & \textcolor{red}{\ding{55}} & 8k \\ \cmidrule(lr){2-8}
%     & SciEval~\cite{sun2024scieval} & Public  datasets & \textcolor{red}{\ding{55}} & Phy., Chem., Bio. & College & \textcolor{red}{\ding{55}} & 15k \\ \cmidrule(lr){2-8}
%     & SciBench~\cite{wang2023scibench} & University exams & \textcolor{green}{\ding{51}} & Phy., Chem., Math & University & \textcolor{red}{\ding{55}} & 2.1k \\ \cmidrule(lr){2-8}
%     & PHYBench~\cite{qiu2025phybench} & Physic exams & \textcolor{green}{\ding{51}} & Phy. & \makecell{High School,\\College,\\Olympiad} & \textcolor{red}{\ding{55}} & 500 \\ \cmidrule(lr){2-8}
%     & SciHorizon~\cite{qin2025scihorizon} & 
%     Public datasets & \textcolor{green}{\ding{51}} & \makecell{Math., Phys., Chem. \\ Bio., Earth \& Space} & College & \textcolor{red}{\ding{55}} & unknown \\ \cmidrule(lr){2-8}
%     & SciRepEval~\cite{singh2022scirepeval} & Scientific literature & \textcolor{red}{\ding{55}} & 20 subjects & Expert & \textcolor{red}{\ding{55}} & 12.4M \\ \cmidrule(lr){2-8}
    
%     & \textbf{Ours} & Scientific literature & \textcolor{green}{\ding{51}} & \makecell{Phy., Chem., Bio., Geo., Math.} & Expert & \textbf{\textcolor{green}{\ding{51}}} & 4.5k \\
% \bottomrule
% \end{tabular}
%  }
% \end{table}


% To position our work in the context of existing research, we review prior efforts across three key areas: scientific QA datasets, benchmarks for scientific QA tasks, and reranking methods that have been explored in RAG-based LLM systems

\subsection{Scientific Question Answering Datasets}
 
Existing QA datasets can be broadly divided into two categories: open-domain and scientific datasets. In open domain, Natural Questions (NQ)~\cite{kwiatkowski2019natural}, TriviaQA~\cite{joshi2017triviaqa}, and WebQuestions~\cite{wang2014overview} have served as popular open-domain QA datasets. 
Furthermore,  HotpotQA~\cite{yang2018hotpotqa} and MuSiQue~\cite{trivedi2022musique} emphasize multi-hop reasoning and complex context synthesis. 
In scientific domains, datasets such as BioASQ~\cite{tsatsaronis2012bioasq} and PubMedQA~\cite{jin2019pubmedqa} target biomedical literature, while MATH~\cite{hendrycks2021measuring} and AquaRat~\cite{ling2017program} evaluate mathematical and procedural reasoning. General science benchmarks, including OpenBookQA~\cite{mihaylov2018can} and ARC~\cite{clark2018think}, construct exam-style questions that combine retrieval and multi-step reasoning.

Sorts of studies~\cite{abdallah2025rankify,jin2024flashrag} shown that question-related context, i.e., external knowledge or facts, can help LLM  generate more reliable and accurate answers. However, except for PubMedQA and BioASQ, most datasets do not provide a large amount of contextual information. They assume that relevant context is already retrieved and do not simulate real-world conditions where the model must reason over partially relevant, noisy, or even misleading documents. This limits their ability to reveal the nuanced performance of retrieval and rerankers.



\begin{table}[htbp]
\centering
\caption{Comparison of SciRerankBench among related datasets, toolkits and benchmarks.}
\vspace{-3mm}
\label{tab:compare_benchmark}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\textbf{Type} & \textbf{Work} & \textbf{\makecell{Source Data}} & \textbf{\makecell{Scientific\\Field}} & \textbf{\makecell{Knowledge\\Level}} & \textbf{\makecell{Rerank\\Oriented}} & \textbf{\makecell{Dataset\\Size}} \\
\midrule
\multirow{6}{*}{Dataset} 
    & NQ~\cite{kwiatkowski2019natural} & Google search log & \textcolor{red}{\ding{55}} & General & \textcolor{red}{\ding{55}} & \makecell{307k (train),\\7.8k (dev/test)} \\ \cmidrule(lr){2-7}
    & HotpotQA~\cite{yang2018hotpotqa} & Wikipedia & \textcolor{red}{\ding{55}} & General & \textcolor{red}{\ding{55}} & 113k \\ \cmidrule(lr){2-7}
    & PubMedQA~\cite{jin2019pubmedqa} & PubMed abstracts & Bio. & Expert & \textcolor{red}{\ding{55}} & \makecell{1k expert,\\61k unlabeled,\\211k generated} \\
\midrule
\multirow{2}{*}{Toolkit} 
    & FlashRAG~\cite{jin2024flashrag} & Public benchmarks & \textcolor{red}{\ding{55}} & General & \textcolor{green}{\ding{51}} & unknown \\ \cmidrule(lr){2-7}
    & rankify~\cite{abdallah2025rankify} & Public benchmarks & \textcolor{red}{\ding{55}} & General & \textcolor{green}{\ding{51}} & unknown \\
\midrule
\multirow{16}{*}{Bench.}
    & CRAG~\cite{yang2024crag} & Web search log & \textcolor{red}{\ding{55}} & General & \textcolor{red}{\ding{55}} & 4.4K \\ \cmidrule(lr){2-7}
    & AGIEval~\cite{zhong2023agieval} & Exams & \makecell{Geo., Bio., His.,Chem., Phy.,\\ Eng., Chi., Math, Law, Log.} & High school & \textcolor{red}{\ding{55}} & 8k \\ \cmidrule(lr){2-7}
    & SciEval~\cite{sun2024scieval} & Public  datasets & Phy., Chem., Bio. & College & \textcolor{red}{\ding{55}} & 15k \\ \cmidrule(lr){2-7}
    & SciBench~\cite{wang2023scibench} & University exams & Phy., Chem., Math & University & \textcolor{red}{\ding{55}} & 2.1k \\ \cmidrule(lr){2-7}
    & PHYBench~\cite{qiu2025phybench} & Physic exams & Phy. & \makecell{High School,\\College,\\Olympiad} & \textcolor{red}{\ding{55}} & 500 \\ \cmidrule(lr){2-7}
    & SciHorizon~\cite{qin2025scihorizon} & 
    Public datasets & \makecell{Math., Phys., Chem. \\ Bio., Earth \& Space} & College & \textcolor{red}{\ding{55}} & unknown \\ \cmidrule(lr){2-7}
    & SciRepEval~\cite{singh2022scirepeval} & Scientific literature & 20 subjects & Expert & \textcolor{red}{\ding{55}} & 12.4M \\ \cmidrule(lr){2-7}
    
    & \textbf{Ours} & Scientific literature & \makecell{Phy., Chem., Bio., Geo., Math.} & Expert & \textbf{\textcolor{green}{\ding{51}}} & 4.5k \\
\bottomrule
\end{tabular}
 }
 \vspace{-6mm}
\end{table}




\subsection{Scientific Question Answering Benchmarks}
Scientific QA benchmarks are widely used to evaluate LLMs.
Recent benchmarks target specific domains, such as APBench~\cite{wu2025apbench}, ChemBench~\cite{mirza2024large}, and PHYBench~\cite{qiu2025phybench}, but offer limited insight into cross-domain generalizability and robustness.


To address the limitations of domain-specific benchmarks, several multidisciplinary QA benchmarks have been proposed.
SciEval~\cite{sun2024scieval}, SciBench~\cite{wang2023scibench}, AGIEval~\cite{zhong2023agieval}, SciRepEval~\cite{singh2022scirepeval}, and SciHorizon~\cite{qin2025scihorizon} evaluate LLMs across diverse scientific domains, task formats, and difficulty levels.
In parallel, Rankify~\cite{abdallah2025rankify} and FlashRAG~\cite{jin2024flashrag} provide modular infrastructures for retrieval, reranking, and generation, enabling reproducible experimentation.
However, existing multidisciplinary benchmarks primarily assess end-to-end QA or representation learning performance, without isolating or systematically evaluating reranking components in RAG pipelines.
Conversely, while Rankify and FlashRAG support reranker evaluation, their datasets are largely grounded in open-domain corpora rather than scientific literature, limiting their applicability to scientific RAG settings.




\subsection{Rerankers in Retrieval-Augmented Generated LLMs}
Rerankers in RAG-LLMs can be categorized into the following architectures. \textit{Dense cross-encoder} rerankers: 
BGE~\cite{chen2024bge}, 
Jina~\cite{jina}, 
BCE~\cite{youdao_bcembedding_2023}, and MXBAI~\cite{rerank2024mxbai}. They compute contextualized relevance scores via bi-sequence encoders and have demonstrated strong performance on various ranking tasks. \textit{Sparse lexical} rerankers: such as 
SPLADE~\cite{formal2021splade} utilizes term-level matching with sparsity constraints to maintain interpretability and alignment with classical information retrieval principles. 
Lightweight alternatives like MiniLM~\cite{wang2020minilm} leverage distilled self-attention mechanisms to reduce inference cost while maintaining reasonable accuracy.
\textit{Late-interaction} rerankers like ColBert~\cite{santhanam2021colbertv2} delay token-level interactions until the scoring stage, offering an efficiency accuracy trade-off suitable for large-scale retrieval.
More recently, \textit{LLM-based} rerankers, such as RankGPT~\cite{sun2023chatgpt}, LLM2Vec~\cite{behnamghader2024llm2vec} 
exploit the reasoning capabilities of large generative models to perform zero-shot or instruction-guided reranking, at the cost of increased computational overhead.
\textit{Sequence-to-sequence} rerankers, such as In-Rank~\cite{zhao2023inrank}, tokenize query-document pairs and employ generative decoding to assess relevance, making them suitable for instruction-driven reranking while not relying on LLMs.
Additionally, \textit{listwise ranking models}: RankT5~\cite{zhuang2023rankt5}, ListT5~\cite{yoon2024listt5}, adopt groupwise learning objectives to optimize the global ordering of candidate contexts. 
Twolar~\cite{baldelli2024twolar} proposes a two-step LLM augmented distillation framework for passage reranking, achieving strong performance by transferring knowledge from powerful LLMs to lightweight student models.
Rank-R1~\cite{zhuang2025rank}  enhances the reasoning capability of document rerankers by introducing a reinforcement learning framework optimized for answer-aware rewards. It directly optimizes reranking performance based on downstream QA accuracy rather than traditional relevance labels. G-RAG~\cite{dong2024don}, a \textit {graph-based reranker} that models semantic and relational connections between retrieved documents using graph neural networks (GNNs). 
\textit{Agent-based rerankers} explicitly formulate the reranking process as a decision-making task. Rearank~\cite{zhang2025rearank} introduces a reasoning agent trained via reinforcement learning to iteratively examine candidate passages and generate a globally optimal ranking. 

However, existing benchmarks do not evaluate these rerankers independently in a reliable way. They are usually designed to evaluate end-to-end RAG systems and assume that the retrieved contexts are already of high quality. This makes it difficult to assess how well a reranker can distinguish relevant from irrelevant or misleading passages, especially in scientific tasks where accuracy, terminology, and reasoning precision are crucial.


